Fictitious Play When Agents Are Not Expected-Utility Maximizers: A Geometric Analysis in $2$-Action Games

Fictitious play (FP) is one of the earliest and most fundamental learning procedures in games, where each agent independently chooses a best response to the empirical distribution of opponents' past actions by maximizing the expected payoff with respect to it. However, learning agents may not always be expected-utility maximizers: they may use nonlinear evaluation functionals to account for the uncertainty induced by the opponents, e.g., via risk measures. In this work, we study nonlinear fictitious play (NL-FP), in which each pure action is evaluated by a general, possibly nonlinear functional of the payoff distribution induced by the opponent's empirical belief. To analyze NL-FP, we first identify a single-crossing property (SCP) of evaluation functionals that preserves the classical geometry of FP in $2\times2$ games. Furthermore, we conduct a novel geometric analysis of the convergence behavior of NL-FP in $2\times2$ games, even when the SCP fails. Beyond $2\times2$ games, we show that the convergence of NL-FP in $2\times n$ ($n\ge3$) games may fail even for continuous-time NL-FP, when the two-action player uses conditional value-at-risk (CVaR) in a $2\times3$ game. In addition, we identify a finite-crossing condition that ensures convergence of the selected continuous-time dynamics and the discrete-time iterates in general $2\times n$ games, which also provides new insights into the global landscape of continuous-time classical FP in such games.

==> fig/fp-geometry-common.tex <==
\definecolor{fpInk}{HTML}{344853}%
\definecolor{fpFlow}{HTML}{82919A}%
\definecolor{fpTeal}{HTML}{007F86}%
\definecolor{fpStable}{HTML}{B45F16}%
\definecolor{fpBlueWash}{HTML}{EEF4FA}%
\definecolor{fpPurpleWash}{HTML}{F5F0F8}%
\definecolor{fpGreenWash}{HTML}{EFF7F2}%
\definecolor{fpGoldWash}{HTML}{FCF6E9}%
\pgfmathsetlengthmacro{\fpUnit}{0.35\textwidth}%
\definecolor{fpEquilibriumWash}{HTML}{F6E9BD}%
\tikzset{
  fp flow/.style={draw=fpFlow,line width=0.45pt,
    postaction={decorate},decoration={markings,
      mark=at position 0.54 with {\arrow{Stealth[length=1.35mm,width=1mm]}}}},
  fp threshold/.style={draw=fpInk!65,line width=0.55pt,densely dashed},
  fp stable/.style={draw=fpStable,line width=1.15pt,
    dash pattern=on 3pt off 1.8pt,postaction={decorate},
    decoration={markings,
      mark=at position 0.40 with {\arrow{Stealth[length=2mm,width=1.5mm]}},
      mark=at position 0.77 with {\arrow{Stealth[length=2mm,width=1.5mm]}}}},
  fp spiral/.style={draw=fpTeal,line width=1.05pt},
  fp spiral arrow/.style={fp spiral,postaction={decorate},
    decoration={markings,
      mark=at position 0.52 with {\arrow{Stealth[length=1.8mm,width=1.3mm]}}}},
  fp equilibrium/.style={circle,draw=white,line width=0.8pt,
    fill=fpInk,inner sep=1.9pt},
  fp key/.style={anchor=west,inner sep=0pt,font=\footnotesize}
}%

\def\fpRay#1#2#3#4#5#6#7#8{%
  \pgfmathsetmacro{\fpDX}{#3-#1}%
  \pgfmathsetmacro{\fpDY}{#4-#2}%
  \pgfmathsetmacro{\fpTX}{ifthenelse(\fpDX>0,
    (#6-#1)/abs(\fpDX),(#1-#5)/abs(\fpDX))}%
  \pgfmathsetmacro{\fpTY}{ifthenelse(\fpDY>0,
    (#8-#2)/abs(\fpDY),(#2-#7)/abs(\fpDY))}%
  \pgfmathsetmacro{\fpT}{min(1,\fpTX,\fpTY)}%
  \pgfmathsetmacro{\fpEndX}{#1+\fpT*\fpDX}%
  \pgfmathsetmacro{\fpEndY}{#2+\fpT*\fpDY}%
  \draw[fp flow] (#1,#2) -- (\fpEndX,\fpEndY);%
}
\def\fpToPure{%
  \pgfmathtruncatemacro{\fpUpper}{\fpEndX+\fpEndY>\fpP+\fpQ}%
  \draw[fp flow] (\fpEndX,\fpEndY) -- (\fpUpper,\fpUpper);%
}
\def\fpCorners{%
  \draw[draw=fpInk,line width=0.75pt] (0,0) rectangle (1,1);
  \node[below left,inner sep=3pt] at (0,0) {$(0,0)$};
  \node[below right,inner sep=3pt] at (1,0) {$(1,0)$};
  \node[above left,inner sep=3pt] at (0,1) {$(0,1)$};
  \node[above right,inner sep=3pt] at (1,1) {$(1,1)$};
}%
\def\fpFrame{%
  \draw[fp threshold] (\fpP,0) -- (\fpP,1);
  \draw[fp threshold] (0,\fpQ) -- (1,\fpQ);
  \fpCorners
  \node[below,inner sep=4pt] at (\fpP,0) {$\bar p$};
  \node[left,inner sep=4pt] at (0,\fpQ) {$\bar q$};
}


==> fig/rho-fp-local.tex <==
\begin{scope}
  \fill[fpGreenWash] (0,.76) rectangle (.24,1);
  \fill[fpGoldWash] (.24,.76) rectangle (.48,1);
  \fill[fpBlueWash] (0,.52) rectangle (.24,.76);
  \fill[fpPurpleWash] (.24,.52) rectangle (.48,.76);
  \draw[fp threshold] (.24,.52) -- (.24,1);
  \draw[fp threshold] (0,.76) -- (.48,.76);
  \draw[fpInk,line width=.75pt] (0,.52) rectangle (.48,1);

  \foreach \p/\q/\u/\v in {
      .38/.63/0/0,.63/.61/0/1,.36/.38/1/0,.63/.36/1/1} {
    \draw[fp flow]
      ({1.2*(\p-.3)},{.52+1.2*(\q-.3)}) --
      ({1.2*(\p+.11*(\u-\p)-.3)},
       {.52+1.2*(\q+.11*(\v-\q)-.3)});
  }

  \foreach \turn [remember=\rhoNext as \rhoTop (initially .69)] in {1,...,6} {
    \pgfmathsetmacro{\rhoLeft}{.25/\rhoTop}
    \pgfmathsetmacro{\rhoBottom}{.25/(1-\rhoLeft)}
    \pgfmathsetmacro{\rhoRight}{1-.25/(1-\rhoBottom)}
    \pgfmathsetmacro{\rhoNext}{1-.25/\rhoRight}
    \ifnum\turn=1\relax
      \tikzset{rho local turn/.style={fp spiral arrow}}
    \else
      \tikzset{rho local turn/.style={fp spiral,line width=.65pt}}
    \fi
    \draw[rho local turn]
      (.24,{.52+1.2*(\rhoTop-.3)}) --
      ({1.2*(\rhoLeft-.3)},.76);
    \draw[rho local turn]
      ({1.2*(\rhoLeft-.3)},.76) --
      (.24,{.52+1.2*(\rhoBottom-.3)});
    \draw[rho local turn]
      (.24,{.52+1.2*(\rhoBottom-.3)}) --
      ({1.2*(\rhoRight-.3)},.76);
    \draw[rho local turn]
      ({1.2*(\rhoRight-.3)},.76) --
      (.24,{.52+1.2*(\rhoNext-.3)});
  }
  \node[rho attractor] at (.24,.76) {};
  \node[anchor=north west,font=\scriptsize,text=fpTeal,
    fill=fpGreenWash,inner sep=1.2pt] at (.015,.985) {Stable};

  \fill[fpGoldWash] (0,.24) rectangle (.24,.48);
  \fill[fpGreenWash] (.24,.24) rectangle (.48,.48);
  \fill[fpPurpleWash] (0,0) rectangle (.24,.24);
  \fill[fpBlueWash] (.24,0) rectangle (.48,.24);
  \draw[fp threshold] (.24,0) -- (.24,.48);
  \draw[fp threshold] (0,.24) -- (.48,.24);
  \draw[fpInk,line width=.75pt] (0,0) rectangle (.48,.48);

  \foreach \p/\q/\u/\v in {
      .425/.575/0/1,.59/.66/0/0,.34/.41/1/1,.575/.425/1/0} {
    \draw[fp flow]
      ({1.2*(\p-.3)},{1.2*(\q-.3)}) --
      ({1.2*(\p+.11*(\u-\p)-.3)},
       {1.2*(\q+.11*(\v-\q)-.3)});
  }
  \draw[white,line width=2.5pt] (0,0) -- (.48,.48);
  \draw[fp stable] (0,0) -- (.24,.24);
  \draw[fp stable] (.48,.48) -- (.24,.24);
  \path[draw=white,line width=.75pt,fill=fpStable]
    (.24,.259) -- (.259,.24) -- (.24,.221) -- (.221,.24) -- cycle;
  \node[anchor=north west,font=\scriptsize,text=fpStable,
    fill=fpGoldWash,inner sep=1.2pt] at (.015,.465) {Saddle};
\end{scope}


==> fig/rho-fp-paths.tex <==
\def\rhoSepOneA{(0.000000,0.437500) -- (0.200000,0.350000)}%
\def\rhoSepOneB{(0.307692,0.000000) -- (0.200000,0.350000)}%
\def\rhoSepTwoA{(0.000000,1.000000) -- (0.200000,0.800000)}%
\def\rhoSepTwoB{(0.400000,0.600000) -- (0.200000,0.800000)}%
\def\rhoSepThreeA{(0.000000,0.583333) -- (0.200000,0.466667) -- (0.400000,0.600000)}%
\def\rhoSepThreeB{(0.416667,1.000000) -- (0.533333,0.800000) -- (0.400000,0.600000)}%
\def\rhoSepFourA{(0.400000,0.600000) -- (0.650000,0.350000)}%
\def\rhoSepFourB{(1.000000,0.000000) -- (0.650000,0.350000)}%
\def\rhoSepFiveA{(0.562500,1.000000) -- (0.650000,0.800000)}%
\def\rhoSepFiveB{(1.000000,0.692308) -- (0.650000,0.800000)}%
\def\rhoCommonStart{(0.290000,0.410000)}%
\def\rhoAttractor{(0.400000,0.350000)}%
\def\rhoContinuousPath{(0.290000,0.410000) -- (0.400000,0.501408) -- (0.581180,0.350000) -- (0.400000,0.240889) -- (0.342506,0.350000) -- (0.400000,0.406839) -- (0.483825,0.350000) -- (0.400000,0.289361) -- (0.365868,0.350000) -- (0.400000,0.384986) -- (0.454526,0.350000) -- (0.400000,0.308013) -- (0.375730,0.350000) -- (0.400000,0.375271) -- (0.440404,0.350000) -- (0.400000,0.317890) -- (0.381170,0.350000) -- (0.400000,0.369778) -- (0.432092,0.350000) -- (0.400000,0.324005) -- (0.384618,0.350000) -- (0.400000,0.366247) -- (0.426617,0.350000) -- (0.400000,0.328164) -- (0.386999,0.350000) -- (0.400000,0.363786) -- (0.422737,0.350000)}%
\def\rhoDiscretePath{(0.290000,0.410000) -- (0.334375,0.446875) -- (0.373529,0.479412) -- (0.408333,0.508333) -- (0.439474,0.481579) -- (0.467500,0.457500) -- (0.492857,0.435714) -- (0.515909,0.415909) -- (0.536957,0.397826) -- (0.556250,0.381250) -- (0.574000,0.366000) -- (0.590385,0.351923) -- (0.605556,0.338889) -- (0.583929,0.326786) -- (0.563793,0.315517) -- (0.545000,0.305000) -- (0.527419,0.295161) -- (0.510937,0.285937) -- (0.495455,0.277273) -- (0.480882,0.269118) -- (0.467143,0.261429) -- (0.454167,0.254167) -- (0.441892,0.247297) -- (0.430263,0.240789) -- (0.419231,0.234615) -- (0.408750,0.228750) -- (0.398780,0.223171) -- (0.389286,0.241667) -- (0.380233,0.259302) -- (0.371591,0.276136) -- (0.363333,0.292222) -- (0.355435,0.307609) -- (0.347872,0.322340) -- (0.340625,0.336458) -- (0.333673,0.350000) -- (0.347000,0.363000) -- (0.359804,0.375490) -- (0.372115,0.387500) -- (0.383962,0.399057) -- (0.395370,0.410185) -- (0.406364,0.420909) -- (0.416964,0.413393) -- (0.427193,0.406140) -- (0.437069,0.399138) -- (0.446610,0.392373) -- (0.455833,0.385833) -- (0.464754,0.379508) -- (0.473387,0.373387) -- (0.481746,0.367460) -- (0.489844,0.361719) -- (0.497692,0.356154) -- (0.505303,0.350758) -- (0.512687,0.345522) -- (0.505147,0.340441) -- (0.497826,0.335507) -- (0.490714,0.330714) -- (0.483803,0.326056) -- (0.477083,0.321528) -- (0.470548,0.317123) -- (0.464189,0.312838) -- (0.458000,0.308667) -- (0.451974,0.304605) -- (0.446104,0.300649) -- (0.440385,0.296795) -- (0.434810,0.293038) -- (0.429375,0.289375) -- (0.424074,0.285802) -- (0.418902,0.282317) -- (0.413855,0.278916) -- (0.408929,0.275595) -- (0.404118,0.272353) -- (0.399419,0.269186) -- (0.394828,0.277586) -- (0.390341,0.285795) -- (0.385955,0.293820) -- (0.381667,0.301667) -- (0.377473,0.309341) -- (0.373370,0.316848) -- (0.369355,0.324194) -- (0.365426,0.331383) -- (0.361579,0.338421) -- (0.357813,0.345313) -- (0.354124,0.352062) -- (0.360714,0.358673) -- (0.367172,0.365152) -- (0.373500,0.371500) -- (0.379703,0.377723) -- (0.385784,0.383824) -- (0.391748,0.389806) -- (0.397596,0.395673) -- (0.403333,0.401429) -- (0.408962,0.397642) -- (0.414486,0.393925) -- (0.419907,0.390278) -- (0.425229,0.386697) -- (0.430455,0.383182) -- (0.435586,0.379730) -- (0.440625,0.376339) -- (0.445575,0.373009) -- (0.450439,0.369737) -- (0.455217,0.366522) -- (0.459914,0.363362) -- (0.464530,0.360256) -- (0.469068,0.357203) -- (0.473529,0.354202) -- (0.477917,0.351250) -- (0.482231,0.348347) -- (0.478279,0.345492) -- (0.474390,0.342683) -- (0.470565,0.339919) -- (0.466800,0.337200) -- (0.463095,0.334524) -- (0.459449,0.331890) -- (0.455859,0.329297) -- (0.452326,0.326744) -- (0.448846,0.324231) -- (0.445420,0.321756) -- (0.442045,0.319318) -- (0.438722,0.316917) -- (0.435448,0.314552) -- (0.432222,0.312222) -- (0.429044,0.309926) -- (0.425912,0.307664) -- (0.422826,0.305435) -- (0.419784,0.303237) -- (0.416786,0.301071) -- (0.413830,0.298936) -- (0.410915,0.296831) -- (0.408042,0.294755) -- (0.405208,0.292708) -- (0.402414,0.290690) -- (0.399658,0.288699) -- (0.396939,0.293537) -- (0.394257,0.298311) -- (0.391611,0.303020) -- (0.389000,0.307667) -- (0.386424,0.312252) -- (0.383882,0.316776) -- (0.381373,0.321242) -- (0.378896,0.325649) -- (0.376452,0.330000) -- (0.374038,0.334295) -- (0.371656,0.338535) -- (0.369304,0.342722) -- (0.366981,0.346855) -- (0.364688,0.350937) -- (0.368634,0.354969) -- (0.372531,0.358951) -- (0.376380,0.362883) -- (0.380183,0.366768) -- (0.383939,0.370606) -- (0.387651,0.374398) -- (0.391317,0.378144) -- (0.394940,0.381845) -- (0.398521,0.385503) -- (0.402059,0.389118) -- (0.405556,0.386842) -- (0.409012,0.384593) -- (0.412428,0.382370) -- (0.415805,0.380172) -- (0.419143,0.378000) -- (0.422443,0.375852) -- (0.425706,0.373729) -- (0.428933,0.371629) -- (0.432123,0.369553) -- (0.435278,0.367500) -- (0.438398,0.365470) -- (0.441484,0.363462) -- (0.444536,0.361475) -- (0.447554,0.359511) -- (0.450541,0.357568) -- (0.453495,0.355645) -- (0.456417,0.353743) -- (0.459309,0.351862) -- (0.462169,0.350000) -- (0.465000,0.348158) -- (0.462565,0.346335) -- (0.460156,0.344531) -- (0.457772,0.342746) -- (0.455412,0.340979) -- (0.453077,0.339231) -- (0.450765,0.337500) -- (0.448477,0.335787) -- (0.446212,0.334091) -- (0.443970,0.332412) -- (0.441750,0.330750) -- (0.439552,0.329104) -- (0.437376,0.327475) -- (0.435222,0.325862) -- (0.433088,0.324265) -- (0.430976,0.322683) -- (0.428883,0.321117) -- (0.426812,0.319565) -- (0.424760,0.318029) -- (0.422727,0.316507) -- (0.420714,0.315000) -- (0.418720,0.313507) -- (0.416745,0.312028) -- (0.414789,0.310563) -- (0.412850,0.309112) -- (0.410930,0.307674) -- (0.409028,0.306250) -- (0.407143,0.304839) -- (0.405275,0.303440) -- (0.403425,0.302055) -- (0.401591,0.300682) -- (0.399774,0.299321) -- (0.397973,0.302477) -- (0.396188,0.305605) -- (0.394420,0.308705) -- (0.392667,0.311778) -- (0.390929,0.314823) -- (0.389207,0.317841) -- (0.387500,0.320833) -- (0.385808,0.323799) -- (0.384130,0.326739) -- (0.382468,0.329654) -- (0.380819,0.332543) -- (0.379185,0.335408) -- (0.377564,0.338248) -- (0.375957,0.341064) -- (0.374364,0.343856) -- (0.372785,0.346624) -- (0.371218,0.349370) -- (0.369665,0.352092) -- (0.372292,0.354792) -- (0.374896,0.357469) -- (0.377479,0.360124) -- (0.380041,0.362757) -- (0.382582,0.365369) -- (0.385102,0.367959) -- (0.387602,0.370528) -- (0.390081,0.373077) -- (0.392540,0.375605) -- (0.394980,0.378112) -- (0.397400,0.380600) -- (0.399801,0.383068) -- (0.402183,0.385516) -- (0.404545,0.383992) -- (0.406890,0.382480) -- (0.409216,0.380980) -- (0.411523,0.379492) -- (0.413813,0.378016) -- (0.416085,0.376550) -- (0.418340,0.375097) -- (0.420577,0.373654) -- (0.422797,0.372222) -- (0.425000,0.370802) -- (0.427186,0.369392) -- (0.429356,0.367992) -- (0.431509,0.366604)}%
\def\rhoDiscretePoints{(0.290000,0.410000),(0.334375,0.446875),(0.373529,0.479412),(0.408333,0.508333),(0.439474,0.481579),(0.467500,0.457500),(0.492857,0.435714),(0.515909,0.415909),(0.536957,0.397826),(0.556250,0.381250),(0.574000,0.366000),(0.590385,0.351923),(0.605556,0.338889),(0.583929,0.326786),(0.563793,0.315517),(0.545000,0.305000),(0.527419,0.295161),(0.510937,0.285937),(0.495455,0.277273),(0.480882,0.269118),(0.467143,0.261429),(0.454167,0.254167),(0.441892,0.247297),(0.430263,0.240789),(0.419231,0.234615),(0.408750,0.228750),(0.398780,0.223171),(0.389286,0.241667),(0.380233,0.259302),(0.371591,0.276136),(0.363333,0.292222),(0.355435,0.307609),(0.347872,0.322340),(0.340625,0.336458),(0.333673,0.350000),(0.347000,0.363000),(0.359804,0.375490),(0.372115,0.387500),(0.383962,0.399057),(0.395370,0.410185),(0.406364,0.420909),(0.416964,0.413393),(0.427193,0.406140),(0.437069,0.399138),(0.446610,0.392373),(0.455833,0.385833),(0.464754,0.379508),(0.473387,0.373387),(0.481746,0.367460),(0.489844,0.361719),(0.497692,0.356154),(0.505303,0.350758),(0.512687,0.345522),(0.505147,0.340441),(0.497826,0.335507),(0.490714,0.330714),(0.483803,0.326056),(0.477083,0.321528),(0.470548,0.317123),(0.464189,0.312838),(0.458000,0.308667),(0.451974,0.304605),(0.446104,0.300649),(0.440385,0.296795),(0.434810,0.293038),(0.429375,0.289375),(0.424074,0.285802),(0.418902,0.282317),(0.413855,0.278916),(0.408929,0.275595),(0.404118,0.272353),(0.399419,0.269186),(0.394828,0.277586),(0.390341,0.285795),(0.385955,0.293820),(0.381667,0.301667),(0.377473,0.309341),(0.373370,0.316848),(0.369355,0.324194),(0.365426,0.331383),(0.361579,0.338421)}%
\def\rhoDiscreteLatePoints{(0.357813,0.345313),(0.397596,0.395673),(0.440625,0.376339),(0.477917,0.351250),(0.455859,0.329297),(0.429044,0.309926),(0.405208,0.292708),(0.383882,0.316776),(0.364688,0.350937),(0.394940,0.381845),(0.422443,0.375852),(0.447554,0.359511),(0.460156,0.344531),(0.441750,0.330750),(0.424760,0.318029),(0.409028,0.306250),(0.394420,0.308705),(0.380819,0.332543),(0.372292,0.354792),(0.392540,0.375605),(0.411523,0.379492),(0.429356,0.367992)}%

